Wave propagation in the frequency regime in one-dimensional quasiperiodic media -Limiting absorption principle

We study the one-dimensional Helmholtz equation with (possibly perturbed) quasiperiodic coefficients. Quasiperiodic functions are the restriction of higher dimensional periodic functions along a certain (irrational) direction. In classical settings, for real-valued frequencies, this equation is generally not well-posed: existence of solutions in L 2 is not guaranteed and uniqueness in L $\infty$ may fail. This is a well-known difficulty of Helmholtz equations, but it has never been addressed in the quasiperiodic case. We tackle this issue by using the limiting absorption principle, which consists in adding some imaginary part (also called absorption) to the frequency in order to make the equation well-posed in L 2 , and then defining the physically relevant solution by making the absorption tend to zero. In previous work, we introduced a definition of the solution of the equation with absorption based on Dirichlet-to-Neumann (DtN) boundary conditions. This approach offers two key advantages: it facilitates the limiting process and has a direct numerical counterpart. In this work, we first explain why the DtN boundary conditions have to be replaced by Robin-to-Robin boundary conditions to make the absorption go to zero. We then prove, under technical assumptions on the frequency, that the limiting absorption principle holds and we propose a numerical method to compute the physical solution.

==> figures.tex <==
% Pour corriger le bug du cercle
\makeatletter
\def\pgfplots@install@path@replacements{%
    \ifpgfplots@path@replace@ellipse
        \let\tikz@do@circle=\pgfplots@path@@tikz@do@circle
        \let\tikz@do@ellipse=\pgfplots@path@@tikz@do@circle
        \expandafter\def\expandafter\pgfinterruptpicture\expandafter{\pgfinterruptpicture
            \let\tikz@do@circle=\pgfplots@path@@tikz@do@circle@orig
            \let\tikz@do@ellipse=\pgfplots@path@@tikz@do@ellipse@orig
        }%
    \fi
}%
\let\pgfplots@path@@tikz@do@circle@orig=\tikz@do@circle
\let\pgfplots@path@@tikz@do@ellipse@orig=\tikz@do@ellipse

\let\pgfplots@path@@tikz@do@circle@oldandbroken=\pgfplots@path@@tikz@do@circle
\def\pgfplots@path@@tikz@do@circle#1{\pgfplots@path@@tikz@do@circle@oldandbroken{#1}{#1}}
\def\pgfplots@path@@tikz@do@ellipse#1#2{\pgfplots@path@@tikz@do@circle@oldandbroken{#1}{#2}}
\makeatother

% Commande \genererFibrage
% 1 : coté du carré
% 2 : abscisse du point de départ de la ligne (relativement au coin inférieur gauche)
% 3 : ordonnée du point de départ de la ligne (relativement au coin inférieur gauche)
% 4 : première composante du vecteur de coupe
% 5 : deuxième composante du vecteur de coupe
% 6 : nombre de composantes de la ligne
% 7 : Longueur de domaine maximale
% 8 : style de tracé
%
% ///////////////////////////////////////////////////////////////////// %
% Attention aux pbs de précision surtout quand on est proche d'un coin. %
% ///////////////////////////////////////////////////////////////////// %
\newcommand{\genererFibrage}[8]{% <-- don't forget this
  \begingroup
    \pgfmathsetmacro\sommetAx{#2}
    \pgfmathsetmacro\sommetAy{#3}
    \pgfmathsetmacro\xextremite{min(#7*#1, (#1 - \sommetAx)/#4, (#1 - \sommetAy)/#5)}
    \pgfmathsetmacro\sommetBx{\sommetAx + \xextremite * #4}
    \pgfmathsetmacro\sommetBy{\sommetAy + \xextremite * #5}
    \pgfmathsetmacro\numIterations{#6-1}
    \pgfmathsetmacro\Lcourante{\xextremite}
    %
    \draw[#8] (\sommetAx, \sommetAy) -- (\sommetBx, \sommetBy);
    %
    % On ne fait la boucle que si la longueur maximale n'est pas encore atteinte
    \pgfmathparse{less(#7*#1, (\Lcourante+0.0001*#1)}
    \ifthenelse{\equal{\pgfmathresult}{0}}{%

      % On ne continue que si le nombre d'itérations est non nul
      \ifdim \numIterations pt > 0pt
      \foreach \idlignes in {1,..., \numIterations} {

      \pgfmathparse{less((#1 - \sommetAx)/#4, (#1 - \sommetAy)/#5)}
      %
      \ifthenelse{\equal{\pgfmathresult}{1}}{%
        \pgfmathsetmacro\nextsommetAx{0}
        \pgfmathsetmacro\nextsommetAy{\sommetBy}
      }{%
        \pgfmathsetmacro\nextsommetAx{\sommetBx}
        \pgfmathsetmacro\nextsommetAy{0}
      }%
      %
      %
      % \ifthenelse{\boolean{#8}}{
      %   \draw[#9] (\sommetBx, \sommetBy) -- (\nextsommetAx, \nextsommetAy);
      % }{}
      \pgfmathsetmacro\nextxextremite{min((#7*#1-\Lcourante), (#1 - \nextsommetAx)/#4, (#1 -\nextsommetAy)/#5)}
      \pgfmathsetmacro\nextsommetBx{\nextsommetAx + \nextxextremite * #4}
      \pgfmathsetmacro\nextsommetBy{\nextsommetAy + \nextxextremite * #5}
      \pgfmathsetmacro\nextLcourante{\Lcourante + \xextremite}
      \draw[#8] (\nextsommetAx, \nextsommetAy) -- (\nextsommetBx, \nextsommetBy);
      %
      %
      % On arrête si la longueur maximale est atteinte
      \pgfmathparse{less(#7*#1, (\nextLcourante+0.0001*#1)}
      \ifthenelse{\equal{\pgfmathresult}{1}}{%
        \breakforeach
      }
      %
      %
      \global\let\sommetAx=\nextsommetAx
      \global\let\sommetAy=\nextsommetAy
      \global\let\sommetBx=\nextsommetBx
      \global\let\sommetBy=\nextsommetBy
      \global\let\xextremite=\nextxextremite
      \global\let\Lcourante=\nextLcourante
      }
      \fi
    }{}

  \endgroup
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Style to select only points from #1 to #2 (inclusive)
\pgfplotsset{select coords between index/.style 2 args={
    x filter/.code={
        \ifnum\coordindex<#1\def\pgfmathresult{}\fi
        \ifnum\coordindex>#2\def\pgfmathresult{}\fi
    }
}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% H1Dlap
% spectres
\pgfplotstableread{DtN_vp_alpha_0_5.txt}\DtNvpA
\pgfplotstableread{DtN_vp_alpha_1.txt}\DtNvpB
\pgfplotstableread{spectre_op_qp.txt}\specDiffOpQP

% Solution 1D
\pgfplotstableread{usol_loc_omega.txt}\uLocPertLAP

% Erreurs
\pgfplotstableread{erreur_omega_eps.txt}\erreursLAP
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Lire un tableau depuis un fichier
\ExplSyntaxOn
\ior_new:N \g_hringriin_file_stream

\NewDocumentCommand{\ReadFile}{mm}
 {
  \hringriin_read_file:nn { #1 } { #2 }
  \cs_new:Npn #1 ##1
   {
    \str_if_eq:nnTF { ##1 } { * }
      { \seq_count:c { g_hringriin_file_ \cs_to_str:N #1 _seq } }
      { \seq_item:cn { g_hringriin_file_ \cs_to_str:N #1 _seq } { ##1 } }
   }
 }

\cs_new_protected:Nn \hringriin_read_file:nn
 {
  \ior_open:Nn \g_hringriin_file_stream { #2 }
  \seq_gclear_new:c { g_hringriin_file_ \cs_to_str:N #1 _seq }
  \ior_map_inline:Nn \g_hringriin_file_stream
   {
    \seq_gput_right:cx
     { g_hringriin_file_ \cs_to_str:N #1 _seq }
     { \tl_trim_spaces:n { ##1 } }
   }
  \ior_close:N \g_hringriin_file_stream
 }

\ExplSyntaxOff

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% \newcommand{\plotmsh}
% Read a file written in the following format
% ------------------------------------------
% number_of_nodes
% index_node,    x_node,    y_node
% number_of_elements
% index_element,   node_1,    node_2,    node_3
% ----------------------------------------------
% Arguments: 1. file name
%            2. nodes color
%            3. elements color
\newcommand{\plotmsh}[3]{
  % \only<1>{
  \ReadFile{\mshelements}{#1}
  % }
  \pgfmathsetmacro\nbnoeuds{\mshelements{1}}
  \pgfmathsetmacro\nbelemts{\mshelements{\nbnoeuds+2}}
  % Draw elements
  \foreach \idI in {1,...,\nbelemts} {
    \pgfmathsetmacro\idsA{{\mshelements{\idI+\nbnoeuds+2}}[1]}
    \pgfmathsetmacro\idsB{{\mshelements{\idI+\nbnoeuds+2}}[2]}
    \pgfmathsetmacro\idsC{{\mshelements{\idI+\nbnoeuds+2}}[3]}
    %
    \draw[#3] ({\mshelements{\idsA+1}}[1], {\mshelements{\idsA+1}}[2])--%
              ({\mshelements{\idsB+1}}[1], {\mshelements{\idsB+1}}[2])--%
              ({\mshelements{\idsC+1}}[1], {\mshelements{\idsC+1}}[2]);
  }
  %
  %
  % Draw nodes
  \foreach \idI in {1,..., \nbnoeuds} {
    \fill[#2] ({\mshelements{\idI+1}}[1], {\mshelements{\idI+1}}[2]) circle[radius=0.5pt];
  }
}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% Plot curve with linear regression
% #1: file ID
% #2: x label
% #3: y label
% #4: plot options for the curve
% #5: plot options for the regression
% #6: relative position of the triangle
% #7: path for triangle slope
% #8: position of the slope label
% #9: name for slope variable
\newcommand{\plotcurveandregression}[9]{%
\addplot [#4] table [x={#2}, y={#3}] {#1};%
\addplot [#5] table [x={#2}, y={create col/linear regression={y={#3}}}] {#1}
              coordinate [pos=#6] (A) % save two points on the regression
              coordinate [pos={#6 + 0.25}] (B); % line for drawing the slope triangle

\xdef#9{\pgfplotstableregressiona} % save the slope parameter
   \draw[#5] (A) #7 (B)  % draw the opposite and adjacent sides of the triangle
      % node [pos=0.25, anchor=south] {1} % label the horizontal line
      node [#8] {\pgfmathprintnumber{#9}}; %label the vertical line
}
